Performance of the Data Handling Hub readout system for the Belle II pixel detector

The SuperKEKB accelerator in Tsukuba, Japan is providing e$^+$e$^-$ beams for the Belle II experiment since March 2019. To deal with the aimed peak luminosity being forty times higher than the one recorded at Belle, a pixel detector based on DEPFET technology has been installed. It features a long integration time of 20 $\mu$s resulting in an expected data rate of 20 GByte/s (160 GBit/s) at a maximum occupancy of 3 %. To deal with this high amount of data, the data handling hub (DHH) has been developed. It contains all necessary functionality for the control and readout of the detector. In this paper we describe the architecture and features of the DHH system. Further we will show the key performance characteristics after one year of operation.

==> references.tex <==
\begin{thebibliography}{00}
\bibitem{DEPFET}
C.~Marinas \emph{et. al},``The Belle II pixel detector: High precision with low material," in \textit{Nucl. Instrum. Meth. A} 731, 31-35 (2013)
\bibitem{DCD}
I.~Peric \emph{et al.} ``DCDB and SWITCHERB, the readout ASICS for Belle II DEPFET
pixel detector," in \textit{Nuclear Science Symposium and Medical Imaging Conference (NSS/MIC)}, Oct 2011, pp. 1536–1539.
\bibitem{DHP}
M.~Lemarenko, T.~Hemperek, H.~Kr\"uger, M.~Koch, F.~L\"utticke, C.~Marinas and N.~Wermes,
``Test results of the data handling processor for the DEPFET pixel vertex detector," in \textit{JINST} 8, C01032 (2013)

\bibitem{Gaisbauer:2016txp}
D.~Gaisbauer, Y.~Bai, I.~Konorov, S.~Paul and D.~Steffen,
``Self-triggering readout system for the neutron lifetime experiment PENeLOPE," \textit{JINST} 11, no.02, C02068 (2016)
\bibitem{GaisbauerUCF}
D.~Gaisbauer \emph{et al.} ``Unified Communication Framework,'' in \textit{IEEE Trans. Nucl. Sci.}, vol. 64, no. 10, Oct. 2017

\bibitem{Nakao:2012zz}
M.~Nakao,
``Timing distribution for the Belle II data acquistion system," \textit{JINST} 7, C01028 (2012)

\bibitem{Frazier:2012iva}
R.~Frazier, G.~Iles, D.~Newbold and A.~Rose,
``Software and firmware for controlling CMS trigger and readout hardware via gigabit Ethernet,"
\textit{Phys. Procedia} 37, 1892-1899 (2012)

\bibitem{Steffen:2018tdp}
D.~Steffen \emph{et al.}
``Intelligence Elements and Performance of the FPGA-based DAQ of the COMPASS Experiment,''
in \textit{TWEPP-17}, 127 (2018)

\bibitem{Spruck:2020voo}
B.~Spruck \emph{et al.} ``Belle II Pixel Detector Commissioning and Operational Experience,'' in \textit{Vertex2019}, Lopud, Croatia, 2020, 015

\bibitem{Bona:2007qt}
M.~Bona \emph{et al.},``SuperB: A High-Luminosity Asymmetric e+ e- Super Flavor Factory. Conceptual Design Report,"[arXiv:0709.0451 [hep-ex]].

\bibitem{Baehr:2015tbf}
S.~Baehr, O.~Sander, M.~Heck, C.~Pulvermacher, M.~Feindt and J.~Becker,
``Online-Analysis of Hits in the Belle-II Pixeldetector for Separation of Slow Pions from Background," in \textit{J. Phys. Conf. Ser.} 664, no.9, 092001 (2015)

\bibitem{ONSEN}
B. Spruck \emph{et al.}, ``The Belle II pixel detector data acquisition and reduction system," in  \textit{IEEE Trans. Nucl. Sci.,} vol. 60, no. 5, pp. 3709–3713, 2013.

\bibitem{EPICS}
Leo R. Dalesio \emph{et.al}, ``The experimental physics and industrial control system architecture: past, present, and future", in \textit{NIMA}, 352, 1-2, pp.179--184, 1994

\bibitem{gatedmode}
M. Valentan, E. Prinker, F. Müller, C. Koffmane and R. Richter, "Gated mode operation of DEPFET sensors for the Belle II pixel detector," in \textit{Nuclear Science Symposium and Medical Imaging Conference (NSS/MIC)},  San Diego, CA, 2015, pp. 1-6
\end{thebibliography}
